Constrainahedra

We define a family of convex polytopes called constrainahedra, which index collisions of horizontal and vertical lines. Our construction proceeds by first defining a poset $C(m,n)$ of good rectangular preorders, then proving that $C(m,n)$ is a lattice, and finally constructing a polytopal realization by taking the convex hull of a certain explicitly-defined collection of points. The constrainahedra will form the combinatorial backbone of the second author's construction of strong homotopy duoids. We indicate how constrainahedra could be realized as Gromov-compactified configuration spaces of horizontal and vertical lines; viewed from this perspective, the constrainahedra include naturally into the first author's notion of 2-associahedra.

==> extras.tex <==
\section{Constrainahedra as generalized permutahedra}

Recall the definition of a generalized permutahedron. 


\begin{defi}
The braid arrangement is a fan whose rays are ...
\end{defi}

\begin{defi}
A generalized permutahedron in the sense of Postnikov is a polytope whose normal fan is coarsening of the braid arrangement.
\end{defi}

We have already done all the work for the following theorem.

\begin{theo}
Constrainahedra are generalized permutahedra.
\end{theo}

\begin{proof}
According to [??], generalized permutahedra are characterized by having edge directions $e_i-e_j$ for some basis vectors. In the proof of Lemma \ref{hyperplane} we have described all the edges, and their directions are just like that.
\end{proof}

For generalized permutahedra, there exists an Ardilla-Doker lifting operation that . Let $P$

\begin{defi}
..
\end{defi}

\begin{theo}
The Ardilla-Doker lift of $C(n_1, \ldots, n_k)$ is $C(n_1, \ldots, n_k,2)$.
\end{theo}

\begin{proof}
Support function
\end{proof}

This is a complicated way to see that $C(2,2, \ldots, 2)$ is always a permutahedron combinatorially. The easy way to see this is to observe that in $\Coll(2,2,\ldots,2)$, all collisions are orthogonal to each other. Thus higher constrainahedra have not only associahedra and multiplihedra as subfamilies, but also permutahedra.

\section{Recursive structure: first thoughts}

Operadically meaningful polytopes always come with some with some recursive structure, i.e. their facets can be described in terms of lower-dimensional analogous polytopes. Consider the following situations.

\begin{itemize}
    \item A face of an associahedron is a product of associahedra. This is a manifestation of the fact that associahedra form an operad.
    \item A face of a multiplihedron is a product of multiplihedra and associahedra. This is a manifestation of the fact that multiplihedra form an operadic bimodule over the operad of associahedra.
    \item A face of a 2-associahedron is a fiber product of 2-associahedra over an associahedron. This is a manifestation of the fact that 2-associahedra form a 2-operad relative to the operad of associahedra.
\end{itemize}

For constrainahedra, the algebraic situation is not yet completely understood. In this section we explain which version of recursive structure is observed polytopally. The answer is as follows: every face of a constrainahedron is a product of some constrainahedra and some {\em grid products} of constrainahedra. Taking a grid product is an operation 
